THE-Pose: Topological Prior with Hybrid Graph Fusion for Estimating Category-Level 6D Object Pose

Category-level object pose estimation requires both global context and local structure to ensure robustness against intra-class variations. However, 3D graph convolution (3D-GC) methods only focus on local geometry and depth information, making them vulnerable to complex objects and visual ambiguities. To address this, we present THE-Pose, a novel category-level 6D pose estimation framework that leverages a topological prior via surface embedding and hybrid graph fusion. Specifically, we extract consistent and invariant topological features from the image domain, effectively overcoming the limitations inherent in existing 3D-GC based methods. Our Hybrid Graph Fusion (HGF) module adaptively integrates the topological features with point-cloud features, seamlessly bridging 2D image context and 3D geometric structure. These fused features ensure stability for unseen or complicated objects, even under significant occlusions. Extensive experiments on the REAL275 dataset show that THE-Pose achieves a 35.8% improvement over the 3D-GC baseline (HS-Pose) and surpasses the previous state-of-the-art by 7.2% across all key metrics. The code is avaialbe on https://github.com/EHxxx/THE-Pose

==> ICCV2025-Author-Kit-Feb/rebuttal_table.tex <==
\begin{table}[h]
\centering
\vspace{-2mm}
\caption{Depth reconstruction results for synthetic sequences.}    
\vspace{-2mm}
    \label{tab:rebutal1}  

\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c|cc|cc}
\hline
\textbf{}  & \multicolumn{2}{c|}{t=0} & \multicolumn{2}{c}{t=1} \\ \cline{2-5} 
\textbf{}     & \multicolumn{1}{c|}{MAE $\downarrow$}             & RMSE $\downarrow$           & \multicolumn{1}{c|}{MAE $\downarrow$}   & RMSE $\downarrow$  \\ \hline
NFL (RAL 23)  & \multicolumn{1}{c|}{0.1699}          & 0.2070          & \multicolumn{1}{c|}{0.1746}                        & 0.2090        \\ \cline{1-5} 
Dex-NeRF (CoRL 21)          & \multicolumn{1}{c|}{0.4019}          & 0.4213          & \multicolumn{1}{c|}{0.4092}                        & 0.4296  \\ \cline{1-5} 
\textbf{Ours} & \multicolumn{1}{c|}{\textbf{0.0419}} & \textbf{0.1059} & \multicolumn{1}{c|}{\textbf{0.0926}}               & \textbf{0.1637} \\ \hline
\end{tabular}
}
\vspace{-4mm}
\end{table}

==> ICCV2025-Author-Kit-Feb/sec/0_abstract_prev.tex <==
\begin{abstract}
3D graph convolution (3D-GC) directly estimates Category-level object pose using only depth information in the image. Excluding visual information enables 3D-GC to handle significant intra-class variation and be robust to color differences. However, the lack of global context and focusing on local structure results in several drawbacks such as being vulnerable to outliers and low performance in the category comprising complex objects. In this paper, we argue that extracting global context in the image could fill the missing piece of 3D-GC.
Hence, we develop the image-based topological prior that includes geometric and topological information and precludes irrelevant color information. Moreover, through our Hybrid Graph Fusion module, we successfully combine the prior's global information and local geometry in point clouds. As a result, our method significantly overcomes the innate limitation of 3D-GC. Extensive experiments on REAL275 demonstrate that our method achieves a significant leap forward over the 3D-GC baseline (HS-Pose) by 35.8\% and outperforms the state-of-the-art by 7.2\% across all key metrics.

% shjeong ver
Category-level object pose estimation requires both global context and local structure to ensure robustness against intra-class variations. However, 3D graph convolution (3D-GC) based methods solely focus on local and depth information. Therefore, their lack of global context cause problems that are vulnerable to complex objects and visual ambiguities. To address this, we define a Topological prior, which effectively filters out irrelevant information from images and satisfies various consistencies beneficial for pose estimation. We extended instance-level SurfEmb to operate at the category level to fulfill this prior, and proposed THE-pose, where the key component is the HGF module, which maximizes the performance of 3D graph convolution by adaptively interpolating between the feature distances extracted from the image-based topological prior and the geometric distances among points. Extensive experiments on REAL275 demonstrate that our method achieves a significant leap forward over the 3D-GC baseline (HS-Pose) by 35.8\% and outperforms the state-of-the-art by 7.2\% across all key metrics.

% Category-level object pose estimation seeks to predict the full 6D pose and 3D size of objects within a given category but remains challenging due to large intra-class shape variations.
% \ak{we don't need definition. just go directly to the point. what is the limitation of current SOTA and how you win over it?}
% Although prior-based methods have shown strong performance, shape priors that rely on mean shapes struggle with significant geometric diversity. 
% \ak{Be more specific to the problem of existing method}
% Similarly, recently introduced semantic priors from vision foundation models often lack essential 3D geometric context and fail to guarantee \(SE(3)\)-invariance. 
% \ak{why semantic and shape prior is inferior to topological prior? this is not intuitive.}
% To address these shortcomings, we propose a novel topological prior that assures geometric consistency, topological consistency, and $SE(3)$-invariance by retraining a category-specific surface embedding, providing a unified latent space for each category. We then integrate this topological prior into our framework via two complementary modules. First, a \emph{Topological Global Context Aggregator} captures robust global features for generalized categorical representations. Second, a \emph{Hybrid Graph Fusion} module combines these topological features with local point cloud features via 3D graph convolution, yielding complementary geometric cues for improved pose estimation. Extensive experiments on REAL275 demonstrate that our method achieves a significant leap forward over the 3D-GC baseline (HS-Pose) by 35.8\% and outperforms the state-of-the-art by 7.2\% across all key metrics.


% datasets demonstrate that THE-Pose achieves robust and accurate 6D pose estimation under significant shape variations and occlusions, substantially improving generalization to unseen instances.

\end{abstract}

==> ICCV2025-Author-Kit-Feb/sec/3_method_prev.tex <==
\section{Methodology}
\label{sec:methods}

\subsection{Overview} 
\label{subsec:overview}
Given an RGB-D image, we first use a segmentation model, such as Mask R-CNN \cite{MaskRcnn}, to obtain each object's segmentation mask and category label. For each segmented object, we extract a cropped RGB image $\mathbf{I}_{\text{obj}} \in \mathbb{R}^{H \times W \times 3}$ and generate a point cloud $\mathcal{P}_{\text{obj}} \in \mathbb{R}^{N \times 3}$ by back-projecting the depth image using camera intrinsics and applying a downsampling process. Using these inputs, THE-Pose predicts the full 6D pose of the object, including 3D rotation $\mathbf{R} \in SO(3)$, 3D translation $\mathbf{t} \in \mathbb{R}^3$, and 3D size $\mathbf{s} \in \mathbb{R}^3$.

The framework of THE-Pose is shown in \hyperref[fig:main-pipeline]{{\underline{\textcolor{blue}{Figure} \textcolor{red}{2}}}}. The method consists of three main components:
i) \textbf{Topological Global Context Aggregator} (\hyperref[subsec:TGC]{{\underline{\textcolor{blue}{Sec.} \textcolor{red}{3.2}}}}), ii) \textbf{Hybrid Graph Fusion module} (\hyperref[subsec:HGF]{{\underline{\textcolor{blue}{Sec.} \textcolor{red}{3.3}}}}), iii) \textbf{Pose\&Size Estimator} (\hyperref[subsec:PSE]{{\underline{\textcolor{blue}{Sec.} \textcolor{red}{3.4}}}}).
Details about each component are provided in the following sections.



% Building on HS-Pose~\cite{HS-Pose}, the final extracted features are passed through three sub-modules for object pose regression, symmetric-based point cloud reconstruction, and bounding box voting in training. During inference, only the encoder and the pose regression module are used.
\subsection{Topological Prior and Global Context}
\label{subsec:TGC}
To ensure versatile intra-class variation while maintaining the primary information of the category, we propose a novel prior called \textbf{Topological Prior}. This prior satisfies three properties as
\begin{itemize}
    \item \textbf{Geometric consistency}: Symmetric surfaces should be represented by identical features.
    \item \textbf{Topological consistency}: Topologically equivalent parts within the category should be encoded with consistent representations.
    \item $\boldsymbol{SE(3)}$ \textbf{invariance} : The prior should remain unaffected by rotation and translation.
\end{itemize}

\noindent These three properties are crucial for category-level 6D pose estimation. For example, let's consider the situation of observing a mug. If the handle is not visible in the scene, the mug loses its cylindrical symmetry and effectively loses one dimension in its 6D pose. The first property is necessary to reflect this change. The second property is essential for achieving accurate feature correspondences between two mugs, enabling the connection of geometric information within the same category. The last property ensures robustness in that the viewpoint or orientation does not influence this representation.

To obtain this potential prior, we utilize the surface embedding method introduced in SurfEmb~\cite{SurfEmb}. This method has the advantage of satisfying geometric consistency and $SE(3)$ invariance. To complete the missing piece, the topological consistency, we retrain this framework to ensure that it has a common latent space across categories by learning on per-category networks. Specifically, we generated synthesized images from 3D models used in only the training set of the existing dataset~\cite{NOCS}. We establish this network as a backbone for obtaining topological prior and freeze both the training and inference stages in the main pipeline.


% To handle the intra-class variation in the main challenge of this task, we use surface embedding for representing \textit{Topological Prior}. 
% In SurfEmb \cite{SurfEmb}, a one-dimensional manifold is used to learn the geometric characteristics of objects, as represented by surface embedding. This is achieved through the learning of 2D-3D correspondence distributions, which encode the relationship between 2D image data and 3D geometric information. Specifically, SurfEmb proposes a method for learning 2D-3D correspondence distributions. In this process, cropped RGB and mask images are fed into an encoder-decoder style query model to generate dense query embeddings, while 3D geometric information is input to a key model. The contrastive learning process then ensures the learning of dense and continuous 2D-3D correspondences. This approach captures the object's surface well, creating a continuous manifold that reflects the surface geometry and maintains the object's intrinsic properties regardless of pose. Additionally, by using the mask image as input, the model demonstrates strong performance even in the presence of occlusions, effectively handling missing parts of the object.


% Building on this concept, we extend it to category-level pose estimation by designing a category-specific network in which objects within the same category share a common latent space. This shared latent space, learned through surface embeddings, not only enables generalization across diverse objects within the category but also provides a topological prior that captures intrinsic geometric properties. By using an SE(3)-invariant surface embedding, our method ensures robust pose estimation, as the learned representations effectively handle large intra-class shape variations.

We retrain the backbone $f_s$ to extract topological embeddings by inputting the cropped object image $\mathbf{I}_{obj}$ and category vector $\mathbf{c}$. This allows the model to learn a latent representation that captures both geometric and topological properties. Given the complexity of object shapes at the category level, a deeper feature representation is necessary to accurately estimate poses. To achieve this, we apply a convolutional layer to further refine the output from $f_s$. This process enables the model to generate high-dimensional feature maps $\mathcal{F}^I_t \in \mathbb{R}^{H \times W \times \mathcal{C}}$ that preserve fine-grained details crucial for accurate category-level pose estimation. The operation is formulated as follows:
\begin{equation}
    \mathcal{F}^I_t = \textit{ConvLayer}(f_s(\mathbf{I}_{obj}, \mathbf{c}))
\end{equation}

Furthermore, the Topological prior captures detailed local features and provides a shared latent space that can effectively represent the global context, essential for addressing complex shape variations. To leverage the advantages of our prior, we use STViT \cite{STViT}, a well-suited vision transformer for capturing global context while preserving detailed local features. Thus, this module takes the topological embedding feature map $ \mathcal{F}^I_t$ as input and, following this, extracts the topological global feature $\mathcal{F}^g_t \in \mathbb{R}^{1 \times \mathcal{D}}$. This topological global context also mitigates the limitations of the 3D-GC network discussed in (\hyperref[subsec:HGF]{{\underline{\textcolor{blue}{Sec.} \textcolor{red}{3.3}}}}).


% Intra-class variations를 해결하기 위한 Topological prior를 얻기 위해, 우리는 2D-3D matching을 통해  Surface embedding을 사용하였다. However, SurfEmb relies on object-specific networks trained using 3D CAD models, limiting its scalability to real-world scenarios with unknown objects. In our work, we adopt a more generalizable approach where we leverage a category-level training approach, enabling the network to generate similar features for objects within the same category rather than assigning an object-specific CAD model. Inspired SurfEmb, 각 카테고리별로 query model과 key model이 있다. query model은 2D image를 input으로 받아 dense query embedding image를 mapping하는 encoder-decoder CNN 이고, key model은 3D point cloud를 input으로 받아 object coordinates를 key embeddings로 mapping하는 MLP이다.  

% \subsection{Topological Global Context Aggregator} 
% \label{subsec:TGC}

% 이 Task에서 complex shape variations를 잘 다루기 위해서는 global context가 필수적인데, Topological Prior로서의 surface embedding은 detailed local feature도 잘 나타내지만, shared latent space를 나타내므로 global context를 잘 표현할 수 있는 장점이 있다. 또한, global context는 complex variations in same category 문제를 해결할 수 있을 뿐만 아니라, Sec3.4에서 사용하는 3D-GC network의 한계점을 해결할 수도 있다. 이를 위해 STViT에 base on 하였는데, 이는 Super Token이라는 시각 토큰 간의 유사성을 기반으로 그룹화하여 이미지의 전역적인 의미와 구조를 효과적으로 나타내는 압축 표현을 소개하였다. 이를 활용하여 self-attention 및 convolution을 적용한 Super Token Blocks를 통해 global context를 effictive하게 포착하면서도, detailed local feature도 capture가 가능하다. 그래서, category-level에 효과적인 global feature를 얻을 수 있다. 그래서, 이 network가 적용된 Global Feature Aggregator module에 surface embedding feature map(H x W x D)이 input으로 들어가 4개의 Super Token Blocks를 거쳐, 1x1 convolution 및 global average pooling을 통해 global feature \(F_g \in \mathbb{R}^{1 \times {D_2}}\)를 얻는다. 



\subsection{Hybrid Graph Fusion} 
\label{subsec:HGF}
% 3D-GC와 receptive field가 왜 이 6D pose에서 중요한 의미를 가지는지 목적을 설명, topological feaeture는 detail이 부족해지는데 이를 detailed geometry로 보완하기 위해 fusion 하였음을 설명.  
\textbf{Hybrid Receptive Field.}
Previous works~\cite{FS-Net, GPV-Pose} demonstrate 3D-GC~\cite{3D-GC}'s capability of perceiving local details by their receptive field and estimating rotation in this field. 

Conventional 3D-GC \cite{3D-GC, FS-Net, GPV-Pose} typically relies on the Euclidean distance between points, limiting the receptive field to local geometric information. In contrast, recent work \cite{HS-Pose} has shown that the receptive field in the feature space can capture geometric relationships over a larger area. 
In our approach, we define a hybrid receptive field (HRF) that combines both point-level and feature-level distances. Since both the surface embedding and the point cloud features inherently capture complementary topological and geometric information, we adopt a weighting factor \(\alpha\) to balance their relative importance. Specifically, we define the hybrid distance between two points \(p_i\) and \(p_j\) as
\begin{equation}
\label{eq3}
D_{\alpha}(i,j) = \alpha\, D_{\text{feat}}(i,j) + (1-\alpha)\, D_{\text{point}}(i,j)
\end{equation}
where $D_{\text{feat}}(i,j)=\|\mathcal{F}_i-\mathcal{F}_j\|$ is the Euclidean distance between their corresponding feature representations and $D_{\text{point}}(i,j)=\|\mathbf{p}_i-\mathbf{p}_j\|$ is the Euclidean distance between the point clouds.
This formulation allows the receptive field to adaptively incorporate both local details and larger geometric relationships, resulting in a more detailed and comprehensive representation.
% Feature based distance로 Partial observations이나 occlusion 상황에서 예측 가능하게 하면서, 정확한 pose 추정을 위한 local detail도 놓치지 않는다.  
\begin{figure}[!t]
  \centering
  \fbox{\rule{0pt}{1.6in} \rule{.6\linewidth}{0pt}}
  \caption{\textbf{Visualize HGF layer by point cloud } }
  \label{fig:stvit-block}
\end{figure}

\noindent \textbf{Fusion Stream}
We propose a 3D graph convolution–based fusion module, termed \textbf{Hybird Graph Module(HGF)} module, composed of stacked \emph{HGF-layers}. Each HGF-layer follows a two-path design analogous to HS-layer \cite{HS-Pose}, ensuring the capture of local and global relationships, scale/translation awareness, and outlier-robust, which are the limitations of previous 3D-GC based methods. 
We first back-propagate the topological feature map  $\mathcal{F}^I_t \in \mathbb{R}^{H \times W \times D_1}$ to obtain  $\mathcal{F}^P_t \in \mathbb{R}^{N \times \mathcal{D}_1}$, which corresponds to the point cloud features. These are then concatenated with  $\mathcal{F}^P_{h,1} \in \mathbb{R}^{N \times \mathcal{D}_2}$, which is extracted from the HGF surface layer using an HRF based only on point distance ($\alpha=0$). The concatenated fusion feature $\mathcal{F}^P_f \in \mathbb{R}^{N \times ({\mathcal{D}_1+\mathcal{D}_2})}$ is used as input to the HGF module for further processing.
% 위 문단에서 글의 순서를 변경. 먼저, 목적을 말하고 우리가 이것을 제안했다고 말하는 순서로. 그리고, HGF surface layer -> 3D GC로 표현 변경, 우리는 HGF module을 제안하는데 전체적인 network 흐름은 HS-pose를 따르고, HGF layer에서 많은 것들을 바꿨다고 주장. 
% First path 설명 전에 이것이 HGF layer 상의 path라고 설명.
In the first path, we perform spatial encoding by applying positional encoding to the fused feature, providing essential spatial information for accurate size and translation estimation.
In the second path, the fused feature  $\mathcal{F}^P_{h,i}$ is passed through a hybrid receptive field that applies more weight to the feature distance, forming graph nodes. These nodes are then enriched with positional encoding and fed into the 3D graph convolution layer. The output is processed using a modified version of outlier robust from \cite{HS-Pose}, where the hybrid receptive field with a stronger emphasis on point distance is applied. This approach enhances robustness to outliers and captures a wider range of spatial geometric relationships, resulting in a more refined feature representation, denoted as \ $\mathcal{F}^P_{h,i+1}$.
Finally, the outputs of these two paths are combined via element-wise summation. Multiple HGF layers are stacked hierarchically, alternated with 3D max-pooling layers, to enhance both local detail and overall geometric consistency gradually. The final layer also outputs the global feature $\mathcal{F}^g_h$, which captures a larger geometric context. Ultimately, the features obtained from all layers are concatenated to form the final fused feature representation:


\begin{equation}
\label{eq4}
 \mathcal{F}^P_f = \mathcal{F}^P_{h,1} \oplus \mathcal{F}^P_{h,2} \oplus \dots \oplus \mathcal{F}^P_{h,5} \oplus \mathcal{F}^g_h.
\
\end{equation}


\subsection{Pose\&Size Estimator} \label{subsec:PSE}

Given the topological global-wise features $\mathcal{F}^g_t \in \mathbb{R}^{N \times \mathcal{D}_t}$ and the hybrid fused feature $\mathcal{F}^P_f \in \mathbb{R}^{N \times \mathcal{D}_f}$, we concatenate them point-wise and directly regress the rotation, as well as the residuals of size and translation. The process is formulated as follows:
\begin{equation}
\label{eq5}
\mathcal{F}_{pose} = \mathcal{F}^g_t \oplus \mathcal{F}^P_f
\end{equation}\begin{equation}
\label{eq6}
R, (t^*, S^*) = MLP_R(F_{pose}), MLP_S(F_{pose} \oplus P_{obj})  
\end{equation}
From \cite{HS-Pose}, we employ a decoupled rotation strategy for rotation estimation and estimate size and translation by predicting the residual size and translation between the ground truth and the mean position and size of the input point cloud. 

We use the extracted features during training to perform object pose regression, symmetric-based point cloud reconstruction, and bounding box voting from \cite{GPV-Pose}. Only the encoder and pose regression modules are employed during inference to predict the final pose and size parameters.


% \subsection{Training and Inference} \label{subsec:estimator}

% Our Pose/Size Estimator follows the architecture used in HS-Pose. The final feature used for pose estimation is obtained by concatenating the semantic global feature extracted in Section with the fusion feature produced by the HGF module in Section. This combined feature is then processed by dedicated regression heads to predict the 6D pose (rotation and translation) and object size.




\vspace{5pt}

% \noindent
% \textbf{Category-specific Surface Embedding}
% Inspired by SurfEmb, we propose a category-specific surface embedding method that maps each surface point $\mathbf{p}\in\mathbb{R}^3$ into a latent space via a function 
% \[
% f: \mathbb{R}^3 \rightarrow \mathbb{R}^d,
% \]
% such that its representation remains invariant under any SE(3) transformation like Fig.1. In our framework, for each point we first extract intrinsic geometric descriptors $\phi(\mathbf{p})$ (e.g., local curvature and geodesic distances) that are inherently independent of the object pose. These descriptors are then fed into a multi-layer perceptron $f$ to produce a $d$-dimensional embedding:
% \[
% \mathbf{z} = f\big(\phi(\mathbf{p})\big).
% \]
% To enforce invariance, we employ a contrastive loss that minimizes the distance between embeddings of corresponding surface points (obtained from different views or under different SE(3) transformations) while maximizing the distance between non-corresponding ones. Furthermore, our embedding network is trained in a category-specific manner to capture discriminative surface properties unique to each object category. This specialized training aligns embeddings across different instances within the same category, ensuring that the latent representation $\mathbf{z}$ remains robust to SE(3) transformations while preserving category-specific semantic and geometric cues.


%%%Previous Intro%%%

% Inspired by the above discussions, we address the limitations of 3D-GC methods by introducing a new type of prior called the \textbf{Topological Prior}. Integrating this prior effectively with point-cloud-based graph convolutions requires reducing unnecessary features while retaining the category's essential information. Conventionally, the image domain was considered unhelpful for existing 3D-GC-based approaches, resulting in minimal attempts at integrating established priors into these methods. 
% In contrast, we introduce a topological prior by extending the surface embedding~\cite{SurfEmb} designed to learn 2D–3D correspondences into the category level. This allows it to provide essential categorical common information from RGB images as a prior, thereby mitigating the insufficient global structure awareness in 3D-GC.



% Motivated by the above discussions, we address the limitations of 3D-GC methods by introducing a new type of prior called the \textbf{Topological Prior}. Integrating this prior effectively with point-cloud-based graph convolutions requires reducing unnecessary features while retaining the category's essential information. Conventionally, the image domain was considered unhelpful for existing 3D-GC-based approaches, resulting in minimal attempts at integrating established priors into these methods. In contrast, we introduce a topological prior by extending the surface embedding~\cite{SurfEmb} designed to learn 2D–3D correspondences into the category level. This allows it to provide essential categorical common information from RGB images as a prior, thereby mitigating the insufficient global structure awareness in 3D-GC. The point requires retraining, the information training.
% Existing priors (i.e., shape and semantic priors) are learned from image domains, resulting in a lack of understanding of geometry. Moreover, their ability to capture detailed features can hinder matching between different objects within the same category as \cref{fig:fig1}. To effectively integrate with point-cloud-based graph convolutions, reducing unnecessary features and retaining only the core information is required. We attain the prior by expanding the surface embedding~\cite{SurfEmb}  to category-level, which possesses potential to capture geometric symmetry and SE3-invariance,

% while overcoming their limitations, we propose a novel type of prior called \textbf{topological prior}

% , satisfying three properties i) geometric consistency, ii) topological consistency, and iii) $SE(3)$-invariance, as illustrated in \cref{fig:fig1}.
% These three properties are particularly important for addressing symmetry ambiguity, intra-class variations, and viewpoint invariance, which are critical challenges in category-level 6D object pose estimation. We attain this prior by retraining the surface embedding framework introduced in SurfEmb~\cite{SurfEmb} in category-level and the details are described at (\hyperref[subsec:TGC]{{\underline{\textcolor{blue}{Sec.} \textcolor{red}{3.2}}}}).
% Our proposed prior is obtained by retraining the categorical surface embedding framework introduced in SurfEmb~\cite{SurfEmb}, enabling it to satisfy both geometric and topological consistency. 
% By doing so, we obtain category-level representations that provide generalized global context while preserving local topological features crucial for effective 3D-GC utilization. 

% By contrast, integrating an $SE(3)$-invariant surface embedding enables more comprehensive local and global features for robust 6D pose estimation even under large shape and color variations in the same categories.


% Recent advancements in category-level 6D pose estimation emphasize the significance of 2D semantic information, with foundation models like DINOv2 demonstrating effective generalization across large datasets [7, 22, 34]. SecondPose uses foundation-model-based semantic priors to address large intra-class shape variations [49]. However, while DINOv2 excels in generalizing object representations across categories, it lacks essential 3D geometric context for category-level pose estimation, particularly in handling complex 3D structures [5, 7]. We tackle this limitation by adopting \emph{surface embeddings} introduced in SurfEmb, which densely encodes an object’s 3D geometry across its surface. Crucially, these embeddings act as a \emph{topological prior} by preserving 3D intrinsic geometric properties and connectivity in an SE(3)-invariant manner, as illustrated in Figure 1. This topological perspective is particularly effective for category-level tasks because surface embeddings generate a unified feature space based on the object’s inherent geometry, even when objects within a category display significant structural variance. As a result, objects with significantly different shapes remain comparable within a shared latent space, offering a robust category-specific representation that accommodates significant intra-class variations.
% building upon HS-Pose~\cite{HS-Pose}

% Shape priors~\cite{SPD}, which represent the mean shape of objects within a category. They obtain correspondence between the object and the prior using RGB features. This prior has the advantage of providing a common standard; however, its performance degrades in instances with significant variations, leading to incorrect correspondences~\cite{AG-Pose}. Recently, SecondPose~\cite{SecondPose} attempted to overcome such limitations by leveraging semantic priors based on a vision foundation model~\cite{DINOv2}. However, there has been insufficient exploration of what constitutes the optimal prior for 6D pose estimation. 

% Recently, alternative type of prior called sementic prior for generalization ablitr
% \ak{Sudden meanwhile and Secondpose blocks the flow.}
% Meanwhile, we have recognized that SecondPose~\cite{SecondPose} employed the vision foundation model DINOv2~\cite{DINOv2} as a semantic prior and demonstrated strong performance. However, as it was trained solely on RGB images, this prior falls short of achieving topological consistency and does not guarantee $SE(3)$-invariance as \figref{fig:fig1}
% \ak{Will we show the result under significant variation? If so, state here.}
% Despite these advancements, category-level object pose estimation still leaves room for improvement.
